Hyperconnected Megacity Parcel Logistic: Joint Parcel Routing and Containerized Consolidation

In high-speed hyperconnected parcel logistics, intermediate hubs play a critical role in reaching economies of scale through consolidating disperse flows of goods. However, resorting small-size parcels at every hub is resource-intensive and can increase hubs' workload and parcels' total travel time. Such resorting can be reduced by smart containerized consolidation, encapsulating together parcels sharing service level and a subsequent destination. In this study, we introduce an optimization model enabling to assess the impact of such consolidation in reducing the expected total pickup-to-delivery times over a parcel logistic network and its consequences on urban logistic operations sustainability. We provide empirical results for a synthetic urban environment, contrasting consolidation performance over different operational and tactical capabilities, network configurations and demand patterns.

==> Results.tex <==
\section{Results} \label{sec:results}


